Stochastic Conditional Gradient Methods: From Convex Minimization to Submodular Maximization

This paper considers stochastic optimization problems for a large class of objective functions, including convex and continuous submodular. Stochastic proximal gradient methods have been widely used to solve such problems; however, their applicability remains limited when the problem dimension is large and the projection onto a convex set is costly. Instead, stochastic conditional gradient methods are proposed as an alternative solution relying on (i) Approximating gradients via a simple averaging technique requiring a single stochastic gradient evaluation per iteration; (ii) Solving a linear program to compute the descent/ascent direction. The averaging technique reduces the noise of gradient approximations as time progresses, and replacing projection step in proximal methods by a linear program lowers the computational complexity of each iteration. We show that under convexity and smoothness assumptions, our proposed method converges to the optimal objective function value at a sublinear rate of $O(1/t^{1/3})$. Further, for a monotone and continuous DR-submodular function and subject to a general convex body constraint, we prove that our proposed method achieves a $((1-1/e)OPT-\eps)$ guarantee with $O(1/\eps^3)$ stochastic gradient computations. This guarantee matches the known hardness results and closes the gap between deterministic and stochastic continuous submodular maximization. Additionally, we obtain $((1/e)OPT -\eps)$ guarantee after using $O(1/\eps^3)$ stochastic gradients for the case that the objective function is continuous DR-submodular but non-monotone and the constraint set is down-closed. By using stochastic continuous optimization as an interface, we provide the first $(1-1/e)$ tight approximation guarantee for maximizing a monotone but stochastic submodular set function subject to a matroid constraint and $(1/e)$ approximation guarantee for the non-monotone case.

==> Algorithm.tex <==
%!TEX root = sample_paper.tex
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%    S  E  C  T  I  O  N   %%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Stochastic Continuous Greedy}\label{sec:scg}
In this section, we introduce our main algorithm, \alg (SCG), which  is a stochastic variant of the continuous greedy method to to solve Problem~\eqref{eq:mainproblem}.
% . Consider the stochastic function $\tilde{F}(\bbx,\bbz): \ccalX \times \reals^m \to \reals_{+} $ where $\bbx \in \ccalX $ is the optimization variable, $\bbz$ is a realization of the random variable $\bbZ$ drawn from from a distribution $P$, and $\ccalX\in \reals^n$ is a compact set. Our goal is to maximize the expectation of the random functions $\tilde{F}(\bbx,\bbz)$ over the convex set $\ccalC$. I.e., we aim to solve the program
%%%%
%\begin{equation}\label{eq:mainproblem}
%OPT\:=\max_{\bbx \in \ccalC}\ F(\bbx) = \max_{\bbx \in \ccalC}\ \mathbb{E}[{\tilde{F} (\bbx,\bbz)}],
%\end{equation}
%%%%
%where the expected function is defined as $F(\bbx):= \mathbb{E}[{\tilde{F} (\bbx,\bbz)}]$. 
We only assume that the expected objective function $F$ is monotone and DR-submodular and the stochastic functions $\tilde{F}(\bbx,\bbz)$ may not be monotone nor submodular. Since the objective function $F$ is monotone and DR-submodular, continuous greedy algorithm \citep{bian16guaranteed,calinescu2011maximizing}  can be used in principle to solve Problem~\eqref{eq:mainproblem}. Note that each update of continuous greedy requires computing the gradient of  $F$, i.e., $\nabla F(\bbx):=\mathbb{E}[{\nabla \tilde{F} (\bbx,\bbz)}]$. However, if we only have access to the (computationally cheap) stochastic gradients ${\nabla \tilde{F} (\bbx,\bbz)}$, then the continuous greedy method will not be directly usable \citep{hassani2017gradient}.  
This limitation is due to the non-vanishing variance of gradient approximations. To resolve this issue, we introduce  stochastic version of the continuous greedy algorithm which reduces the noise of gradient approximations via a common averaging technique in stochastic optimization \citep{ruszczynski1980feasible,ruszczynski2008merit,yang2016parallel,mokhtari2017large}. 

%However, here we assume that the distribution $P$ is either unknown or the domain of the random variable $\bbZ$ is very large which makes the cost of computing the expectation very high. In this regime, resorting to stochastic methods which operate on computationally cheap estimates of gradients arises as a natural solution. Thus, we aim to solve the optimization problem in \eqref{eq:mainproblem} only by using stochastic gradients ${\nabla \tilde{F} (\bbx,\bbz)}$ of the expected objective function $F$. 
%
%It is known that the vanilla stochastic implementation of the Frank-Wolfe algorithm might diverge in convex programs [\red{add citations}] and consequently the continuous greedy method with stochastic gradients $\nabla \tilde{F}(\bbx_t,\bbz_t)$ cannot achieve the optimal approximation factor $1-1/e$ in submodular maximization \citep{hassani2017gradient}. 
%This limitation is due to non-vanishing variance of gradient approximations. To resolve this issue, we introduce a stochastic version of the continuous greedy algorithm which reduces the noise of gradient approximation via a common averaging technique in stochastic optimization \citep{ruszczynski1980feasible,ruszczynski2008merit,yang2016parallel,mokhtari2017large}. 

Let $t \in  \mathbf{N}$ be a discrete time index and $\rho_t$ a given stepsize which approaches zero as $t$ approaches infinity. Our proposed estimated gradient $\bbd_t$ is defined by the following recursion  
%%%%
%%%
\begin{equation} \label{eq:von1}
\bbd_t = (1-\rho_t) \bbd_{t-1} + \rho_t \nabla \tilde{F}(\bbx_t,\bbz_t),
\end{equation}
%%%
%%%%
where the initial vector is defined as $\bbd_0=\bb0$. It can be shown that the averaging technique in \eqref{eq:von1} reduces the noise of gradient approximation as time increases. More formally, the expected noise of gradient estimation $\E{\|\bbd_t-\nabla F(\bbx_t)\|^2}$ approaches zero asymptotically (Lemma~\ref{lemma:bound_on_grad_approx_sublinear}). This property implies that the gradient estimate $\bbd_t$ is a better candidate for approximating the gradient $\nabla F(\bbx_t)$ comparing to the the unbiased gradient estimate $\nabla \tilde{F}(\bbx_t,\bbz_t)$ that suffers from a high variance approximation. We therefore define the  ascent direction $\bbv_t$ of our proposed SCG method as follows
%
%
%can replace the estimate $\bbd_t$ for the unbiased gradient estimate $\nabla \tilde{F}(\bbx_t,\bbz_t)$ \textcolor{red}{replace with $\nabla F$, right?} in the update of the continuous greedy method. Applying this substitution, the update of the ascent direction $\bbv_t$ can be written as
%%%%
\begin{equation}\label{eq:von2}
\bbv_t =\argmax_{\bbv\in \ccalC} \{ \bbd_t^T\bbv \},
\end{equation}
%%%%
which is a linear objective maximization over the convex set $\ccalC$. Indeed, if instead of the gradient estimate $\bbd_t$ we use the exact gradient $\nabla F(\bbx_t)$ for the updates in~\eqref{eq:von2}, the continuous greedy update will be recovered. Here, as in continuous greedy, the initial decision vector is the null vector, $\bbx_0=\bb0$. Further, the stepsize for updating the iterates is equal to $1/T$, and the variable $\bbx_t$ is updated as
%%%
\begin{equation}\label{eq:von3}
\bbx_{t+1} =  \bbx_{t} + \frac{1}{T} \bbv_t.
\end{equation}
%%%
The stepsize $1/T$ and the initialization $\bbx_0=\bb0$ ensure that after $T$ iterations the variable $\bbx_T$ ends up in the convex set $\ccalC$. We should highlight that the convex body $\ccalC$ may not be down-closed or contain $\bb0$. Nonetheless, the solution $\bbx_T$ returned by SCG will be a feasible point in $\ccalC$. 
%(\red{note that we assume $\ccalC$ to be down closed, i.e., $\bb0 \in \ccalC$})
%Also, note that our proposed method is called \alg (SCG) since it can be interpreted as the stochastic variant of the continuous greedy algorithm. 
The steps of the proposed SCG method are outlined in Algorithm \ref{algo_SCGGA}. 





%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%   A   L   G   O   R   I   T   H   M    %%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
\begin{algorithm}[tb]
\caption{\alg (SCG)}\label{algo_SCGGA} 
\begin{algorithmic}[1] 
{\REQUIRE Stepsizes $\rho_t>0$. Initialize $\bbd_0=\bbx_0=\bb0$
%
\FOR {$t=1,2,\ldots, T$}
   \STATE Compute $\bbd_t = (1-\rho_t) \bbd_{t-1} + \rho_t \nabla \tilde{F}(\bbx_t,\bbz_t)$;
   \STATE Compute $\bbv_t =\argmax_{\bbv\in \ccalC} \{ \bbd_t^T\bbv \}$;
   \STATE Update the variable $\bbx_{t+1} =\bbx_{t} + \frac{1}{T} \bbv_t$;
\ENDFOR}
\end{algorithmic}\end{algorithm}


==> abstract.tex <==
%!TEX root = sample_paper.tex
\begin{abstract}
In this paper, we study the problem of \textit{constrained} and \textit{stochastic} continuous submodular maximization. Even though the objective function is not concave (nor convex) and is defined in terms of an expectation, we develop a variant of the conditional gradient method, called \alg, which achieves a \textit{tight} approximation guarantee. More precisely, for a monotone and continuous DR-submodular function and subject to a \textit{general} convex body constraint, we prove that \alg achieves a $[(1-1/e)\text{OPT} -\eps]$ guarantee (in expectation) with   $\mathcal{O}{(1/\eps^3)}$ stochastic gradient computations. This guarantee matches the known hardness results and closes the gap between deterministic and stochastic continuous submodular maximization. By using stochastic continuous optimization as an interface, we also provide the first $(1-1/e)$ tight approximation guarantee for maximizing  a \textit{monotone but stochastic} submodular \textit{set} function subject to a general matroid constraint. 
%More precisely, for a monotone and DR-submodular function, we show that a stochastic conditional gradient method  achieves a $[(1-e^{-1})\text{OPT} -\eps]$ guarantee (in expectation) with   $\mathcal{O}{(1/\eps^3)}$ stochastic gradient computations for 
%
%
%Even though the objective function is stochastic (and is defined in terms of an expectation) and  not concave (nor convex), we show that a stochastic conditional gradient method achieves a $[(1-e^{-1})\text{OPT} -\eps]$ guarantee with   $\mathcal{O}{(1/\eps^3)}$ stochastic gradient computations. 
%
%study
%
%
% the problem of \textit{stochastic} continuous submodular maximization where the objective function is defined in terms of an expectation over an unknown distribution. Even though the object function is not concave (nor convex) we show that a stochastic conditional gradient method provides a \textit{tight} approximation guarantee. More precisely, for a monotone and DR-submodular function  subject to a general  convex body, we prove that by averaging over the stochastic estimates of the gradients, a conditional gradient method  achieves a $[(1-e^{-1})\text{OPT} -\eps]$ approximation (in  expectation) with   $\mathcal{O}{(1/\eps^3)}$ stochastic gradient computations. Our positive result matches known hardness results and closes the gap between deterministic and stochastic submodular maximization by showing that the approximation factor $(1-{e}^{-1})$ is also  achievable in stochastic settings.
% It is well-known that even deterministic DR-submodular functions cannot be 
%
%
%Such stochastic problems  usually arise  from observing data from some data-generating process. 
%
%
%provide the first  stochastic continuous submodular maximization and provide the first 
%
%that  is expressed as an expectation 
%In this paper, we study stochastic submodular maximization where the goal is to maximize a submodular function that can be written as the expected value of  a set of random functions. To solve this class of problems we present a stochastic conditional gradient method which approximates the gradient of the expected objective functions by averaging over the stochastic estimates of its gradients. We show that the 
%iterates generated by the proposed method after $\mathcal{O}{(1/\eps^3)}$ iterations, i.e., $\mathcal{O}{(1/\eps^3)}$ stochastic gradient computations, reach a solution which achieves objective value exceeding $((1-e^{-1})\text{OPT} -\eps)$ in expectation. This result closes the gap between deterministic and stochastic submodular maximization by showing that the approximation factor $(1-e^{-1})$ is achievable for stochastic submodular maximization.
\end{abstract}

==> my_sections.tex <==
\usepackage{needspace}

% \nbsubsubsection{} provides a numbered subsection in bold without a line break. The section will contain at least three lines of text before a pagebreak
\newcommand{\nbsubsubsection}[1]{\needspace{1\baselineskip}\color{white}\subsubsection{#1}\vspace{-3\baselineskip}\color{black}\bigskip{\noindent \bf \thesubsubsection. #1.}}

% \myparagraph provides a paragraph title in italics. 
\newcommand{\myparagraph}[1]{\needspace{1\baselineskip}\medskip\noindent {\it #1.}}

% \myparagraphtc provides a paragraph title in italics. It adds an enter to the table of contents
\newcommand{\myparagraphtc}[1]{\needspace{1\baselineskip}\medskip\noindent {\it #1.}\addcontentsline{toc}{subsubsection}{\qquad\qquad\quad#1}}


